Signatures of microscopic black holes and extra dimensions at future neutrino telescopes

In scenarios with large extra dimensions (LEDs), the fundamental Planck scale can be low enough that collisions between high-energy particles may produce microscopic black holes. High-energy cosmic neutrinos can carry energies much larger than a PeV, opening the door to a higher energy range than Earth-based colliders. Here, for the first time, we identify a number of unique signatures of microscopic black holes as they would appear in the next generation of large-scale neutrino observatories such as IceCube-Gen2 and the Pacific Ocean Neutrino Explorer. These signatures include new event topologies, energy distributions, and unusual ratios of hadronic-to-electronic energy deposition, visible through Cherenkov light echos due to delayed neutron recombination. We find that the next generation of neutrino telescopes can probe LEDs with a Planck scale up to 6 TeV, though the identification of unique topologies could push their reach even further.

==> jdefs.tex <==
% Bibliography and bibfile
\def\pdu{Phys.\ Dark Univ.}
          % Physics of the Dark Universe
\def\lnp{Lec.\ Notes in Physics}
          % Lecture Notes in Physics
\def\cpc{Comp.\ Phys.\ Comm.}
          % Computer Physics Communications
\def\jpg{J. Phys. G}
          % Journal of Physics G Nuclear Physics
\def\ijmpa{Int.\ J.\ Mod.\ Phys.\ A}
          % International Journal of Modern Physics A
\def\epjc{Eur.\ Phys.\ J.\ C}
          % European Physical Journal C
\def\nima{Nuc.\ Inst.\ Methods A}
          % Nuclear Instruments and Methods A
\def\nimb{Nuc.\ Inst.\ Methods B}
          % Nuclear Instruments and Methods B
\def\njp{New J.\ Phys.}
          % New Journal of Physics
\def\rmp{Rev.\ Mod.\ Phys.}
          % Reviews of Modern Physics
\def\app{Astropart.\ Phys.}
          % Astroparticle Physics
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\arnps{Ann.~Rev.~Nucl.~\& Part.~Sci.}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.\ Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\pos{PoS}%
          % Proceedings of Science
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull.\ Astr.\ Inst.\ Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia
\def\caa{Chinese Astron.\ Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J.\ Astron.\ Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jhep{JHEP}%
          % Journal of High Energy Physics
\def\jcap{JCAP}%
          % Journal of Cosmology and Astroparticle Physics
\def\jinst{JINST}%
          % Journal of Instrumentation
\def\jpsj{J.\ Phys.\ Soc.\ Japan}%
          % Journal of the Physical Society of Japan
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\canjphys{Can.~J.~Phys.}
          %Canadian Journal of Physics
\def\apphys{Astropart.~Phys.}
          %Astroparticle Physics
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.\ Rev.\ A}%
          % Physical Review A: General Physics
\def\prb{Phys.\ Rev.\ B}%
          % Physical Review B: Solid State
\def\prc{Phys.\ Rev.\ C}%
          % Physical Review C
\def\prd{Phys.\ Rev.\ D}%
          % Physical Review D
\def\pre{Phys.\ Rev.\ E}%
          % Physical Review E
\def\prx{Phys.\ Rev.\ X}%
          % Physical Review X
\def\prl{Phys.\ Rev.\ Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.\ Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.\ Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\science{Science}%
\def\sci{\science}%
          % Science
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.\ Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.\ Space~Phys.\ Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.\ Astron.\ Inst.\ Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.\ Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.\ Cosmochim.\ Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.\ Res.\ Lett.}%
          % Geophysics Research Letters
\def\jcp{J.\ Chem.\ Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.\ Geophys.\ Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.\ Quant.\ Spec.\ Radiat.\ Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.\ Soc.\ Astron.\ Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.\ Phys.\ A}%
          % Nuclear Physics A
\def\nphysb{Nucl.\ Phys.\ B}%
          % Nuclear Physics B
\def\physrep{Phys.\ Rep.}%
          % Physics Reports
\def\physscr{Phys.\ Scr}%
          % Physica Scripta
\def\planss{Planet.\ Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.\ SPIE}%
          % Proceedings of the SPIE
\def\repprogphys{Rep.\ Prog.\ Phys.}%
          % Reports of Progress in Physics
\def\jpcrd{J. Phys. Chem. Ref. Data}%
        %Journal of Physical and Chemical Reference Data
\def\jphysb{J. Phys. B}%
	%Journal of Physics B Atomic Molecular Physics
\def\jphysd{J. Phys. D}%
	%Journal of Physics D
\def\jphysconfseries{J. Phys. Conf. Series}%
	%Journal of Physics: Conference Series
\def\physrev{\pr}
\def\pr{Phys. Rev.}%
	%Physical Review
\def\josa{J. Opt. Soc. Amer. (1917-1983)}%
	%Journal of the Optical Society of America (1917-1983)
\def\josab{J. Opt. Soc. Amer. B}%
	%Journal of the Optical Society of America B Optical Physics
\def\pla{Phys. Lett. A}%
	%Physics Letters A
\def\plb{Phys. Lett. B}%
	%Physics Letters B
\def\os{Opt. Spectrosc. (Russ.)}%
	%Optics and Spectroscopy (Russ. / USSR)
\def\jas{J. Appl. Spectrosc.}%
	%Journal of Applied Spectroscopy (Russ. / USSR)
\def\annp{Ann. Phys.}%
	%Annalen der Physik
\def\sa{Spectrochim. Acta}%
	%Spectrochimica Acta
\def\prsoca{Proc. R. Soc. London Ser. A}%
	%Proceedings of the Royal Society of London, Series A
\def\zphysa{Z. Phys. A}%
	%Zeitschrift fur Physik A
\def\zphysb{Z. Phys. B}%
	%Zeitschrift fur Physik B
\def\zphysc{Z. Phys. C}%
	%Zeitschrift fur Physik C
\def\zphysd{Z. Phys. D}%
	%Zeitschrift fur Physik D
\def\zphyse{Z. Phys. E}%
	%Zeitschrift fur Physik E
\def\zphys{Z. Phys.}%
	%Zeitschrift fur Physik
\def\adndt{Atom. Data Nuc. Data Tables}%
	%Atomic Data and Nuclear Data Tables
\def\jmolspec{J. Mol. Spectrosc.}%
	%Journal of Molecular Spectroscopy
\def\aphysb{Appl. Phys. B}%
	%Applied Physics B: Lasers and Optics
\def\nim{Nuc. Inst. Meth.}%
	%Nuclear Instruments and Methods
\def\jphysique{J. Phys. (Paris)}%
	%Journal de Physique
\def\epjp{Eur.~Phys.~J.~Plus}%
        %European Physical Journal Plus
\def\epjc{Eur.~Phys.~J.~C}%
        %European Physical Journal C
\def\epl{Europhys.~Lett}%
        %Europhysics Letters
\def\njp{New J.~Phys.}
        %New Journal of Physics
\def\statsci{StatSci}
\def\an{AstNach}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%


